Charged Particle Tracking with Machine Learning on FPGAs

The determination of charged particle trajectories (tracking) in collisions at the CERN Large Hadron Collider (LHC) is one of the most important aspects for event reconstruction at hadron colliders. This is especially true in the high conditions expected during the future high-luminosity phase of the LHC (HL-LHC) where the number of interactions per beam crossing will increase by a factor of five. Deep learning algorithms have been successfully applied to this task for offline applications. However, their study in hardware-based trigger applications has been limited . In this paper, we study different algorithms for two different steps of tracking and show that such algorithms can be run on field-programmable gate arrays (FPGAs).

==> tex/stubcreation.tex <==
\textcolor{red}{Will}

The first step of track reconstruction is the formation of hit clusters from raw hit data, the goal being to group adjacent hits and average their positions to result in one coordinate per detector layer.
In dual-layer strip detectors, these clusters are then combined into spacepoints, taking into account the stereo angle between the closely-spaced layers to give a more precise $z$ coordinate, while in pixel detectors the clusters directly become spacepoints with no combination \textbf{(I think, find a tracking paper though Also, probably cite some things for this)}

To reduce the number of strip spacepoints processed in downstream algorithms, a simple filtering known as \textit{stub finding} can be performed on the relative angular displacement of the strip centres, since the largest such displacements predominantly result from low-\pt tracks.
This is described in \textbf{[a stub reference].}

A common first step in track reconstruction from these spacepoints, and one used as a basis for the work described here, is the creation of first pairs and then triplets of spacepoints compatible with tracks above a given $p_T$ (and hence below a given curvature) originating from the known beamspot $z_0$ and desired $d_0$. 
The constraints on compatibility with a given track $\eta$ and maximum curvature are sufficient to reduce the number of possible triplet candidates to a manageable number, making them a reasonable starting point for more complex track seeding algorithms such as the one described below.
\textbf{quote TDR numbers}


